A Characterization of the Combined Effects of Overlap and Imbalance on the SVM Classifier

In this paper we demonstrate that two common problems in Machine Learning---imbalanced and overlapping data distributions---do not have independent effects on the performance of SVM classifiers. This result is notable since it shows that a model of either of these factors must account for the presence of the other. Our study of the relationship between these problems has lead to the discovery of a previously unreported form of "covert" overfitting which is resilient to commonly used empirical regularization techniques. We demonstrate the existance of this covert phenomenon through several methods based around the parametric regularization of trained SVMs. Our findings in this area suggest a possible approach to quantifying overlap in real world data sets.

==> quantifying-overlap/quantifying-overlap.tex <==
\section{Towards a Quantification of Overlap}
\label{sec:quantifying-overlap}

The original motivation for our work here is not only to study the effects of
overlap but also to explore potential methods for measuring it.  In principle
the problem is ill posed; since we define overlapping regions as areas of the
data space where the (true) class posterior \note{prior? Which am I using?}
probabilities are nearly equal, which means that measurement of these regions
degrades to density estimation; however, since we lack access to these
distributions in real data we must pursue a different approach.

Although our findings are insufficient to formulate a robust measure of overlap,
they do suggest a general method for approaching the problem.  When the classes
are separable we should to be able to detect overfitting by looking at the
generalization performance.  As we have shown, this expectation fails to hold in
cases where the classes overlap.  In this case maximizing the generalization
performance has the effect of localizing any overfitting to the ambiguous
regions, but does not remove it entirely.  In this case it should be possible to
exploit the fact that the artifacts of overfitting will be localized in the
region we wish to measure.  Since we are able to localize the covert overfitting
to the ambiguous (\ie overlapped) regions of the data space we can attempt to
quantify the level of overlap by measuring how overfit we can force the model to
be while still maintaining good generalization performance.

We would like to (covertly) overfit as much as possible to avoid underestimating
the level of overlap, which implies that we want to extremalise the model
parameters.  In the case of an SVM with an RBF kernel, this corresponds to
making $C$ as large as possible and $\gamma$ as small as possible under the
constraint that we achieve good generalization performance.

Secondly, it is important that the model have sufficient representational
capacity to encode the overfit boundary.  This means that models which are
restricted to very simple boundaries (\eg linear models) are not good candidates
for this problem, as it is quite likely that the true boundary contains more
complexity than the model can represent.  Since the techniques we looked at
focus on tracking various statistics as the overfit model is regularized, it is
necessary that the model be capable of overfitting in the first place.  This can
only occur if the representational capacity of the model is greater than the
complexity of the optimal boundary.  The RBF kernel allows an SVM to learn a
model of unbounded complexity, making it an ideal candidate in this respect.

With these criteria we might approach this problem by measuring a quantity
similar to the sufficiency point, which was defined in
Section~\ref{sec:co-results}.  The sufficiency point corresponds (in a somewhat
vague way) to the number of support vectors required to achieve good performance
on the test domain.  In light of this we might propose to measure the degree of
overlap as the ratio between the sufficiency point and the number of essential
support vectors in the original model.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../ol.ib-denil-jmlr"
%%% End: 

